FastSR-NeRF: Improving NeRF Efficiency on Consumer Devices with A Simple Super-Resolution Pipeline

Super-resolution (SR) techniques have recently been proposed to upscale the outputs of neural radiance fields (NeRF) and generate high-quality images with enhanced inference speeds. However, existing NeRF+SR methods increase training overhead by using extra input features, loss functions, and/or expensive training procedures such as knowledge distillation. In this paper, we aim to leverage SR for efficiency gains without costly training or architectural changes. Specifically, we build a simple NeRF+SR pipeline that directly combines existing modules, and we propose a lightweight augmentation technique, random patch sampling, for training. Compared to existing NeRF+SR methods, our pipeline mitigates the SR computing overhead and can be trained up to 23x faster, making it feasible to run on consumer devices such as the Apple MacBook. Experiments show our pipeline can upscale NeRF outputs by 2-4x while maintaining high quality, increasing inference speeds by up to 18x on an NVIDIA V100 GPU and 12.8x on an M1 Pro chip. We conclude that SR can be a simple but effective technique for improving the efficiency of NeRF models for consumer devices.

==> tables/ablation_augmentation.tex <==
\begin{table}
    \begin{center} 
    \resizebox{0.95\columnwidth}{!}{ 
    \begin{tabular}{ ccccc }
        \toprule[1.5pt]
        Dataset & DataAug & PSNR & SSIM & LPIPS \\
        \midrule[0.5pt] 
        \multirow{5}{*}{NeRF Synthetic} 
        & None & 29.01 & 0.931 & 0.086 \\
        & Random Rotation 10$^{\circ}$ \\
        & Random HFlip 10\% \\
        & Random Perspective \\
        & Random Patching & \textbf{30.47} & \textbf{0.944} & \textbf{0.075} \\
        % \midrule[0.5pt] 
        % \multirow{3}{*}{LLFF} & Regular & \ding{55} & 24.65 & 0.748 & \textbf{0.325} \\
        % & Random & \ding{55} & \textbf{24.83} & \textbf{0.750} & 0.328 \\
        % & Random & \ding{51} & 24.70 & 0.745 & 0.336 \\
        \bottomrule[1.5pt]
    \end{tabular}}
    \end{center}
    \caption{Ablation study on data augmentation. The output resolution is 800x800 for NeRF Synthetic dataset, and 1008x756 for LLFF dataset. The upsampling ratio for the super resolution module is 4x.}
    \label{table:abalation_patch_aug}
\end{table}


==> tables/ablation_patch_aug.tex <==
\begin{table}
    \begin{center} 
    \resizebox{0.95\columnwidth}{!}{ 
    \begin{tabular}{ cccccc }
        \toprule[1.5pt]
        Dataset & Patch & DataAug? & PSNR & SSIM & LPIPS \\
        \midrule[0.5pt] 
        \multirow{3}{*}{NeRF Synthetic} & Regular & \ding{55} & 29.01 & 0.931 & 0.086 \\
        & Random & \ding{55} & 29.66 & 0.9365 & \textbf{0.083} \\
        & Random(6/19) & \ding{55} & \textbf{30.47} & \textbf{0.944} & \textbf{0.075} \\
        & Random & \ding{51} & \textbf{30.26} & \textbf{0.942} & 0.085 \\
        \midrule[0.5pt] 
        \multirow{3}{*}{LLFF} & Regular & \ding{55} & 24.65 & 0.748 & \textbf{0.325} \\
        & Random & \ding{55} & \textbf{24.83} & \textbf{0.750} & 0.328 \\
        & Random & \ding{51} & 24.70 & 0.745 & 0.336 \\
        \bottomrule[1.5pt]
    \end{tabular}}
    \end{center}
    \caption{Ablation study on patch sampling algorithms and data augmentation. The output resolution is 800x800 for NeRF Synthetic dataset, and 1008x756 for LLFF dataset. The upsampling ratio for the super resolution module is 4x.}
    \label{table:abalation_patch_aug}
\end{table}


==> tables/ablation_train_strategies.tex <==
\begin{table}
    \begin{center} 
    \resizebox{0.95\columnwidth}{!}{ 
    \begin{tabular}{ ccccc }
        \toprule[1.5pt]
        Upsample & Upsample & Train & Train & \multirow{2}{*}{PSNR} \\
        Ratio & Method & Strategy & Time(m) & \\
        \midrule[0.5pt] 
        \multirow{5}{*}{2x} 
        & Bilinear & - & \textbf{11} & 29.77 \\
        & \multirow{4}{*}{EDSR} 
        & Pretrained & \textbf{11} &  30.40 \\
        & & Scratch & 51 & 31.64 \\
        & & Finetune & 51 & 31.84 \\
        % & & Ours & \textbf{80} & \textbf{32.19} \\
        & & Ours & 89 & \textbf{32.53} \\
        % & & Distillation & 365 & 32.12 \\
        \midrule[0.5pt] 
        \multirow{5}{*}{4x} 
        & Bilinear & - & \textbf{3.5} & 26.67 \\
        & \multirow{4}{*}{EDSR} 
        & Pretrained & \textbf{3.5} & 27.62 \\
        % & & Finetune* & 9.2 & 29.01 \\
        & & Scratch & 19 & 29.03 \\
        & & Finetune & 19 & 29.28 \\
        % & & Ours & \textbf{32} & \textbf{30.12} \\
        & & Ours & 30 & \textbf{30.47} \\
        % & & Distillation & 166 & 29.94\\
        \bottomrule[1.5pt]
    \end{tabular}}
    \end{center}
    \caption{Training time and PSNRs of different training strategies on NeRF Synthetic dataset. (Finetune uses regular patch sampling.) All experiments train for 150 epochs except distillation. *training converged at epoch 60. For distillation training, we generate 1k extra training image using a teacher TensoRF model. The time includes training the teacher model, rendering extra training images, and training the student model.}
    \label{table:abalation_train_strategies}
\end{table}

% 2x finetune: https://bolt.apple.com/tasks/xqdm5fn2ef/
% 2x ours: https://bolt.apple.com/tasks/i5eedd7nhf/


==> tables/depres.tex <==
\begin{table}
    \begin{center} 
    \resizebox{0.99\columnwidth}{!}{ 
    \begin{tabular}{ cc|cc|cc| }
        \toprule[1.5pt]
        Upsample & \multirow{2}{*}{Method} & \multicolumn{2}{|c|}{NeRF Synthetic} & \multicolumn{2}{|c|}{LLFF} \\
        Ratio & & Train Time & PSNR & Train Time & PSNR \\
        % \multirow{2}{*}{\textbf{Method}} & \textbf{Upsample} & \textbf{Train} & \multirow{2}{*}{\textbf{PSNR}} & \multirow{2}{*}{\textbf{SSIM}} & \multirow{2}{*}{\textbf{LPIPS}} & \textbf{Render} & \textbf{Model} \\
        % & \textbf{Ratio} & \textbf{Time} & & & & \textbf{Time(s)} & \textbf{Size(MB)} \\
        \midrule[1pt] 
        \multirow{4}{*}{2} & Bilinear & 18m & 29.77 \\
         & Naive &  &  \\
         & Distillation &  110m & 32.12 \\
         & Data Aug & 80m & 32.19  \\
        \midrule[1pt] 
        \multirow{4}{*}{4} & Bilinear & 18m & 26.67 \\
         & Naive &  &  \\
         & Distillation & 101m & 29.94 \\
         & Data Aug & 32m & 30.124 \\
        \bottomrule[1.5pt]
    \end{tabular}}
    \end{center}
    \caption{Training time and PSNR for different training strategies. The backbone NeRF used here is TensoRF.}
\end{table}

\begin{table}
    \begin{center} 
    \resizebox{0.99\columnwidth}{!}{ 
    \begin{tabular}{ ccc|cc|cc| }
        \toprule[1.5pt]
        Upsample & Upsample & Train & \multicolumn{2}{|c|}{NeRF Synthetic} & \multicolumn{2}{|c|}{LLFF} \\
        Ratio & Method & Strategy & Train Time & PSNR & Train Time & PSNR \\
        % \multirow{2}{*}{\textbf{Method}} & \textbf{Upsample} & \textbf{Train} & \multirow{2}{*}{\textbf{PSNR}} & \multirow{2}{*}{\textbf{SSIM}} & \multirow{2}{*}{\textbf{LPIPS}} & \textbf{Render} & \textbf{Model} \\
        % & \textbf{Ratio} & \textbf{Time} & & & & \textbf{Time(s)} & \textbf{Size(MB)} \\
        \midrule[1pt] 
        \multirow{4}{*}{2} & Bilinear & - & 18m & 29.77 \\
        & \multirow{4}{*}{EDSR} & Pretrained &  &  \\
        & & Finetune &  &  \\
        & & Distillation &  110m & 32.12 \\
        & & Data Aug & 80m & 32.19  \\
        \midrule[1pt] 
        \multirow{4}{*}{4} & Bilinear & & 18m & 26.67 \\
        & \multirow{4}{*}{EDSR} & Pretrained &  &  \\
        & & Finetune &  &  \\
        & & Distillation & 101m & 29.94\\
        & & Data Aug & 32m & 30.124 \\
        \bottomrule[1.5pt]
    \end{tabular}}
    \end{center}
    \caption{Training time and PSNR for different training strategies. The backbone NeRF used here is TensoRF.}
\end{table}

\begin{table}
    \begin{center} 
    \resizebox{0.9\columnwidth}{!}{ 
    \begin{tabular}{ cc|cc|cc| }
        \toprule[1.5pt]
        Upsample & Train & \multicolumn{2}{|c|}{NeRF Synthetic} & \multicolumn{2}{|c|}{LLFF} \\
        Method & Strategy & Train Time & PSNR & Train Time & PSNR \\
        \midrule[1pt] 
        Bilinear & - & 18m & 29.77 \\
        \midrule[0.5pt] 
        \multirow{4}{*}{EDSR} & Pretrained &  &  \\
        & Finetune &  &  \\
        & Distillation &  110m & 32.12 \\
        & Data Aug & 80m & 32.19  \\
        \bottomrule[1.5pt]
    \end{tabular}}
    \end{center}
    \caption{Training time and PSNR of different training strategies for 2X super resolution rate. The backbone NeRF used here is TensoRF.}
\end{table}


==> tables/grid_vs_random_patch.tex <==
\begin{table}[htbp]
% \begin{wrapfigure}{r}{0.85\columnwidth}
    % \begin{center} 
    \centering
    \small
    \resizebox{0.95\columnwidth}{!}{ 
    \begin{tabular}{ cccc }
        \toprule[1.5pt]
        \multirow{2}{*}{Dataset} & \multirow{2}{*}{Method} & \multicolumn{2}{c}{PSNR} \\
        & & SR-2X & SR-4X \\
        % & Ratio & & & & Time(m) & Time(ms) & Size(MB) \\
        \midrule[0.5pt] 
        \multirow{2}{*}{NeRF-Synthetic} 
        & Grid-based & 31.84 & 29.28\\
        & Random & \textbf{32.53} & \textbf{30.47} \\
        \hline
        % \midrule[0.5pt] 
        \multirow{2}{*}{NSVF-Synthetic} & Grid-based & 34.34 & 30.45 \\
        & Random & \textbf{35.39} & \textbf{32.04} \\
        \hline
        % \midrule[0.5pt] 
        \multirow{2}{*}{LLFF} & Grid-based & \textbf{26.2} & 24.94 \\
        & Random & 26.04 & \textbf{25.41} \\
        \bottomrule[1.5pt]
    \end{tabular}
    }
    % \end{center}
    \caption{PSNR comparison on using random patch sampling versus grid-based patch sampling. We highlight the better results for the same SR ratio in \textbf{bold}.}
    \label{table:grid_vs_random_patch}
    % \vspace*{-\baselineskip}
    \vspace{-2em}
% \end{wrapfigure}
\end{table}

==> tables/llff_table.tex <==
\begin{table*}
    \begin{center} 
    \resizebox{0.7\textwidth}{!}{ 
    \begin{tabular}{ ccccccc }
        \toprule[1.5pt]
        \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{PSNR}} & \multirow{2}{*}{\textbf{SSIM}} & \multirow{2}{*}{\textbf{LPIPS}} & \textbf{Train} & \textbf{Render} & \textbf{Model} \\
        & & & & \textbf{Time} & \textbf{Time(s)} & \textbf{Size(MB)} \\
        \midrule[1pt] 
        NeRF & 26.5 & 0.811 & 0.250 & \textcolor{red}{$\sim$2days} & \textcolor{red}{33} & 5 \\
        TensoRF & \colorbox{YellowGreen}{26.6} & 0.832 & 0.207 & 28m & \textcolor{red}{5.9} & \textcolor{red}{188} \\
        \hline
        SNeRG & 25.63 & 0.818 & \colorbox{SkyBlue}{0.183} & \textcolor{red}{$\sim$2days} & 0.036 & \textcolor{red}{310}\\
        MobileNeRF & 25.91 & 0.825 & \colorbox{SkyBlue}{0.183} & \textcolor{red}{$>$2days} & 0.0029 & \textcolor{red}{201.5} \\
        NeX & \colorbox{Yellow}{27.26} & \colorbox{YellowGreen}{0.904} & \colorbox{YellowGreen}{0.178} & \textcolor{red}{20h} & 0.0033 & - \\
        Plenoxel & 26.29 & 0.839 & 0.210 & 24m & - & \textcolor{red}{19300} \\
        % \midrule[1pt] 
        \hline
        MobileR2L & 26.15 & \colorbox{Yellow}{0.966} & 0.187 & \textcolor{red}{$>$2days} & - & 8.3 \\
        NeRF-SR & \colorbox{Yellow}{27.26} & 0.842 & \colorbox{Yellow}{0.103} & \textcolor{red}{$>$2days} & \textcolor{red}{39.1} & - \\ 
        RefSR-NeRF & 26.23 & \colorbox{SkyBlue}{0.874} & 0.243 & - & \textcolor{red}{8.5} & 38 \\
        Ours (2X) & 26.20 & 0.822 & 0.241 & \textbf{150m} & \textbf{0.786} & \textbf{26} \\
        Ours (4X) & 25.41 & 0.784 & 0.297 & \textbf{59m} & \textbf{0.163} & \textbf{15} \\
        % Ours (8X) & 21.30 & 0.584 & 0.475 & \textbf{15m} & \textbf{0.04} & \textbf{8} \\
        \bottomrule[1.5pt]
    \end{tabular}}
    \end{center}
    \caption{Results on real-world forward facing LLFF Datset. Resolution is at 1008x756. The first, second, and third best results of the quality metrics are highlighted in yellow, green and blue. We use red text color when there is a clear disadvantage on either training time, rednering time or model size.}
    \label{table:llff_main}
\end{table*}


==> tables/macbook_training.tex <==
\begin{table}[H]
    \centering
    \resizebox{0.9\columnwidth}{!}{ 
    \begin{tabular}{ ccccc }
        \toprule[1.5pt]
        \multirow{2}{*}{Method} & Train & \multirow{2}{*}{PSNR} & Render & Render Time \\
        & Time & & Time(s) & Speedup \\
        \midrule[0.5pt] 
        % TensoRF & 35m & 32.67 & 37.4 & -\\
        % Ours & 166m & 27.9 & 1.2 & 31x\\
        % \hline
        % \multirow{3}{*}{TensoRF} & 39m & 28.3 & \multirow{3}{*}{54} & \multirow{3}{*}{-} \\
        % & 79m & 32.30 & & \\
        % & 118m & 33.61 & & \\
        \multirow{3}{*}{TensoRF} & 40m & 28.3 & \multirow{3}{*}{54} & \multirow{3}{*}{-} \\
        & 1.3h & 32.30 & & \\
        & 2h & 33.61 & & \\
        \hline
        \multirow{2}{*}{Ours} & 4h & 30.26 & \multirow{2}{*}{3.6} & \multirow{2}{*}{15x} \\
        & 13h & 31.27 & & \\
        \hline
        MobileNeRF & \textcolor{red}{$>$375h} & 30.26 & 0.013 & \\
        \bottomrule[1.5pt]
    \end{tabular}
    }
    \caption{PSNR and time profiling when runing TensoRF and our method on a MacBook Pro laptop with M1 Pro chip. }
    \label{table:macbook_training}
\end{table}

\begin{table}[htbp!]
    \centering
    \resizebox{0.9\columnwidth}{!}{ 
    \begin{tabular}{ cccc }
        \toprule[1.5pt]
        \multirow{2}{*}{Method} & Train & \multirow{2}{*}{PSNR} & Render \\
        & Time & & Time(s) \\
        \midrule[0.5pt] 
        % TensoRF & 35m & 32.67 & 37.4 & -\\
        % Ours & 166m & 27.9 & 1.2 & 31x\\
        % \hline
        % \multirow{3}{*}{TensoRF} & 39m & 28.3 & \multirow{3}{*}{54} \\
        % & 79m & 32.30 & \\
        % & 118m & 33.61 & \\
        \multirow{3}{*}{TensoRF} & 40m & 28.3 & \multirow{3}{*}{54} \\
        & 1.3h & 32.30 & \\
        & 2h & 33.61 & \\
        \hline
        \multirow{2}{*}{TF + SR} & 4h & 30.26 & \multirow{2}{*}{3.6} \\
        & 13h & 31.27 & \\
        \hline
        MobileNeRF & \textcolor{red}{$>$375h}$^{\dagger}$ & 30.26 & 0.013 \\
        \bottomrule[1.5pt]
    \end{tabular}
    }
    \caption{PSNR and time profiling when runing TensoRF and our method on a MacBook Pro laptop with M1 Pro chip. ${\dagger}$ The training time is approximated for training original NeRF, which is the only first training stage of MobileNeRF.}
    \label{table:macbook_training}
\end{table}

==> tables/nerf_synthetic_table.tex <==
\begin{table*}
    \begin{center} 
    \resizebox{0.7\textwidth}{!}{ 
    \begin{tabular}{ ccccccc }
        \toprule[1.5pt]
        \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{PSNR}} & \multirow{2}{*}{\textbf{SSIM}} & \multirow{2}{*}{\textbf{LPIPS}} & \textbf{Train} & \textbf{Render} & \textbf{Model} \\
        & & & & \textbf{Time} & \textbf{Time(s)} & \textbf{Size(MB)} \\
        \midrule[1pt] 
        NeRF & 31.01 & 0.947 & 0.081 & \textcolor{red}{$\sim$35h} & \textcolor{red}{20} & 5 \\
        NSVF$^{\ddagger}$ & 31.74 & 0.953 & \colorbox{SkyBlue}{0.047} & \textcolor{red}{$>$48h} & \textcolor{red}{3} & - \\
        MipNeRF & \colorbox{SkyBlue}{33.09} & \colorbox{SkyBlue}{0.961} & \colorbox{YellowGreen}{0.043} & \textcolor{red}{$\sim$35h} & - & - \\
        % \midrule[1pt] 
        \hline
        KiloNeRF$^{\dagger}$ & 31.00 & 0.950 & \colorbox{Yellow}{0.030} & \textcolor{red}{$>$35h} & 0.026 & - \\
        MobileNeRF$^{\dagger}^{\ddagger}$ & 30.90 & 0.947 & 0.062 & \textcolor{red}{$>$35h} & 0.0013 & \textcolor{red}{125.8} \\
        Plenoxel$^{\dagger}$ &  31.71 & 0.958 & 0.049 & 11m & 0.066 & \textcolor{red}{815} \\
        TensoRF & \colorbox{Yellow}{33.14} & \colorbox{YellowGreen}{0.963} & 0.049 & 18m & \textcolor{red}{1.4} & \textcolor{red}{71.8} \\
        DVGO & 31.95 & 0.957 & 0.053 & 22m & \textbf{TODO} & \textcolor{red}{612} \\
        Instant-NGP$^{\dagger}$ & \colorbox{YellowGreen}{33.18} & - & - & 5m & \textbf{TODO} & 16\\
        % PlenOctrees & 31.71 & 0.958 & 0.053 & \textcolor{red}{$\sim$15h} & 0.006 & \textcolor{red}{1.97(GB)} \\ 
        % FastNeRF & 29.90 & 0.937 & 0.056 & - & 0.041 & \textcolor{red}{$>$7GB} \\
        % SNeRG & 30.38 & 0.950 & 0.05 & \textcolor{red}{$\sim$35h} & 0.012 & \textcolor{red}{86.8} \\
        \hline
        MobileR2L & 31.34 & \colorbox{Yellow}{0.993} & 0.051 & \textcolor{red}{$>$35h} & - & 8.3\\
        NeRF-SR & 28.46 & 0.921 & 0.076 & \textcolor{red}{$>$35h} & 5.6 & - \\
        Ours (2X) & 32.53 & \colorbox{SkyBlue}{0.961} & 0.052 & \textbf{89m} & \textbf{0.309} & \textbf{20} \\
        Ours (4X) & 30.47 & 0.944 & 0.075 & \textbf{30m} & \textbf{0.077} & \textbf{13} \\
        % Ours (8X) & 27.27 & 0.902 & 0.142 & \textbf{16.5m} & \textbf{0.03} & \textbf{8}
        \bottomrule[1.5pt]
    \end{tabular}}
    \end{center}
    \caption{
        Results on NeRF Synthetic Datset. The first section includes models that use a big MLP to represent the radiance field. The middle section includes efficient models that use an explicit or hybrid representation to accelerate both training and inference. The third section collects methods that utilize SR to improve both quality and speed including ours.  Our method achieves a great balance between training time, rendering speed and model size with on par accuracy against other efficient NeRF models. 
        The first, second, and third best results of the quality metrics are highlighted in yellow, green and blue. We use red text color when there is a clear disadvantage on either training time, rednering time or model size.
        $\dagger$ notes the method relies on customized CUDA kernels for the speed, while other methods are based on standard PyTorch framework.
        $\ddagger$ notes the method requires at least 8 high-end GPUs to train.
        % Note: Mip-NeRF training time is an early-stop version on RTX2080Ti GPU. Original training time is longer. Plenoxel uses customized CUDA. MobileNeRF need 8 V100 GPUs to train. 
    }
    \label{table:nerf_synthetic_main}
\end{table*}


==> tables/nsvf_synthetic_table.tex <==
\begin{table*}
    \begin{center} 
    \resizebox{0.7\textwidth}{!}{ 
    \begin{tabular}{ ccccccc }
        \toprule[1.5pt]
        \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{PSNR}} & \multirow{2}{*}{\textbf{SSIM}} & \multirow{2}{*}{\textbf{LPIPS}} & \textbf{Train} & \textbf{Render} & \textbf{Model} \\
        & & & & \textbf{Time} & \textbf{Time(s)} & \textbf{Size(MB)} \\
        \midrule[1pt] 
        NeRF & 30.81 & 0.952 & - & \textcolor{red}{$\sim$35h} & \textcolor{red}{$\sim$20} & $\sim$5 \\
        NSVF$^{\ddagger}$ & 35.13 & \colorbox{Yellow}{0.979} & - & \textcolor{red}{$>$48h} & \textcolor{red}{$\sim$3} & - \\
        \hline
        KiloNeRF & 33.37 & 0.970 & \colorbox{Yellow}{0.020} & \textcolor{red}{$>$35h} & 0.026 & - \\
        DVGO & \colorbox{SkyBlue}{35.18} & \colorbox{Yellow}{0.979} & TODO & $\sim$20m & - & \textcolor{red}{$\sim$600} \\
        TensoRF & \colorbox{Yellow}{36.52} & 0.959 & \colorbox{YellowGreen}{0.027} & 15m & \textcolor{red}{1.4} & \textcolor{red}{74} \\
        \hline
        Ours (2X) & \colorbox{YellowGreen}{35.39} & \colorbox{Yellow}{0.979} & \colorbox{SkyBlue}{0.032} & \textbf{92m} & \textbf{0.302} & \textbf{26} \\
        Ours (4X) & 32.04 & 0.958 & 0.059 & \textbf{30m} & \textbf{0.075} & \textbf{12} \\
        \bottomrule[1.5pt]
    \end{tabular}}
    \end{center}
    \caption{
        Results on NSVF Synthetic Datset. NSVF requires 8 GPUs to train. The first, second, and third best results of the quality metrics are highlighted in yellow, green and blue. We use red text color when there is a clear disadvantage on either training time, rednering time or model size.
        $\ddagger$ notes the method requires at least 8 high-end GPUs to train.
    }
    \label{table:nerf_synthetic_main}
\end{table*}


==> tables/quantitative_results.tex <==
\begin{table*}
    \begin{center}
    % NeRF-Synthetic results
    \begin{subtable}[t]{0.85\textwidth}
        \centering
        \begin{tabular}{ ccccccc }
        \toprule[1.5pt]
        \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{PSNR$\uparrow$}} & \multirow{2}{*}{\textbf{SSIM$\uparrow$}} & \multirow{2}{*}{\textbf{LPIPS$\downarrow$}} & \textbf{Train} & \textbf{Render} & \textbf{Model} \\
        & & & & \textbf{Time} & \textbf{Time(s)} & \textbf{Size(MB)} \\
        \midrule[1pt] 
        NeRF & 31.01 & 0.947 & 0.081 & \textcolor{red}{$\sim$35h} & \textcolor{red}{20} & 5 \\
        NSVF$^{\ddagger}$ & 31.74 & 0.953 & \colorbox{SkyBlue}{0.047} & \textcolor{red}{$>$48h} & \textcolor{red}{3} & - \\
        MipNeRF & \colorbox{SkyBlue}{33.09} & \colorbox{SkyBlue}{0.961} & \colorbox{Yellow}{0.043} & \textcolor{red}{$\sim$35h} & - & - \\
        % \midrule[1pt] 
        \hline
        KiloNeRF$^{\pmb{\dagger}}$ & 31.00 & 0.950 & \colorbox{YellowGreen}{0.030} & \textcolor{red}{$>$35h} & \textbf{0.026} & - \\
        SNeRG & 30.38 & 0.950 & 0.05 & \textcolor{red}{$\sim$35h} & 0.012 & \textcolor{red}{86.8} \\
        MobileNeRF$^{\pmb{\dagger}}$$^{\ddagger}$ & 30.90 & 0.947 & 0.062 & \textcolor{red}{$>$35h} & \textbf{0.0013} & \textcolor{red}{125.8} \\
        DVGO & 31.95 & 0.958 & 0.053 & 14m & \textbf{0.44} & \textcolor{red}{612} \\
        TensoRF & \colorbox{Yellow}{33.14} & \colorbox{Yellow}{0.963} & 0.049 & 18m & \textcolor{red}{1.4} & \textcolor{red}{71.8} \\
        Plenoxel$^{\pmb{\dagger}}$ &  31.71 & 0.958 & 0.049 & 11m & \textbf{0.066} & \textcolor{red}{815} \\
        % DVGOv2$^{\pmb{\dagger}}$ & 32.76 & 0.962 & 0.046 & 7m & 0.254 & \textcolor{red}{612} \\
        Instant-NGP$^{\pmb{\dagger}}$ & \colorbox{YellowGreen}{33.18} & - & - & 5m & - & \textbf{16} \\
        % PlenOctrees & 31.71 & 0.958 & 0.053 & \textcolor{red}{$\sim$15h} & 0.006 & \textcolor{red}{1.97(GB)} \\ 
        % FastNeRF & 29.90 & 0.937 & 0.056 & - & 0.041 & \textcolor{red}{$>$7GB} \\
        \hline
        MobileR2L & 31.34 & \colorbox{YellowGreen}{0.993} & 0.051 & \textcolor{red}{$>$35h} & - & \textbf{8.3} \\
        NeRF-SR & 28.46 & 0.921 & 0.076 & \textcolor{red}{$>$35h} & 5.6 & - \\
        Ours (2X) & 32.53 & \colorbox{SkyBlue}{0.961} & 0.052 & \textbf{89m} & \textbf{0.309} & \textbf{20} \\
        % Ours (4X) & 30.47 & 0.944 & 0.075 & \textbf{30m} & \textbf{0.077} & \textbf{13} \\
        % Ours (8X) & 27.27 & 0.902 & 0.142 & \textbf{16.5m} & \textbf{0.03} & \textbf{8}
        \bottomrule[1.5pt]
        \end{tabular}
        \caption{NeRF Synthetic Dataset results.}
        \vspace{5pt}
    % }
    \end{subtable}
    % NSVF-Synthetic results
    \begin{subtable}[t]{0.85\textwidth}
        \centering
        \begin{tabular}{ ccccccc }
            \toprule[1.5pt]
            \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{PSNR$\uparrow$}} & \multirow{2}{*}{\textbf{SSIM$\uparrow$}} & \multirow{2}{*}{\textbf{LPIPS$\downarrow$}} & \textbf{Train} & \textbf{Render} & \textbf{Model} \\
            & & & & \textbf{Time} & \textbf{Time(s)} & \textbf{Size(MB)} \\
            \midrule[1pt] 
            NeRF & 30.81 & 0.952 & - & \textcolor{red}{$\sim$35h} & \textcolor{red}{$\sim$20} & \textbf{$\sim$5} \\
            NSVF$^{\ddagger}$ & 35.13 & \colorbox{YellowGreen}{0.979} & - & \textcolor{red}{$>$48h} & \textcolor{red}{$\sim$3} & - \\
            \hline
            KiloNeRF$^{\pmb{\dagger}}$ & 33.37 & 0.970 & \colorbox{YellowGreen}{0.020} & \textcolor{red}{$>$35h} & \textbf{0.026} & - \\
            DVGO & \colorbox{SkyBlue}{35.18} & \colorbox{YellowGreen}{0.979} & - & $\sim$20m & - & \textcolor{red}{$\sim$600} \\
            TensoRF & \colorbox{YellowGreen}{36.52} & 0.959 & \colorbox{Yellow}{0.027} & 15m & \textcolor{red}{1.4} & \textcolor{red}{74} \\
            \hline
            Ours (2X) & \colorbox{Yellow}{35.39} & \colorbox{YellowGreen}{0.979} & \colorbox{SkyBlue}{0.032} & \textbf{92m} & \textbf{0.302} & \textbf{26} \\
            % Ours (4X) & 32.04 & 0.958 & 0.059 & \textbf{30m} & \textbf{0.075} & \textbf{12} \\
            \bottomrule[1.5pt]
        \end{tabular}
        \caption{NSVF Synthetic Dataset results.}
        \vspace{5pt}
    \end{subtable}
    \begin{subtable}[t]{0.85\textwidth}
        \centering
        \begin{tabular}{ ccccccc }
            \toprule[1.5pt]
            \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{PSNR$\uparrow$}} & \multirow{2}{*}{\textbf{SSIM$\uparrow$}} & \multirow{2}{*}{\textbf{LPIPS$\downarrow$}} & \textbf{Train} & \textbf{Render} & \textbf{Model} \\
            & & & & \textbf{Time} & \textbf{Time(s)} & \textbf{Size(MB)} \\
            \midrule[1pt] 
            NeRF & 26.5 & 0.811 & 0.250 & \textcolor{red}{$\sim$48h} & \textcolor{red}{33} & \textbf{5} \\
            \hline
            SNeRG & 25.63 & 0.818 & \colorbox{SkyBlue}{0.183} & \textcolor{red}{$\sim$48h} & \textbf{0.036} & \textcolor{red}{310}\\
            NeX & \colorbox{YellowGreen}{27.26} & \colorbox{Yellow}{0.904} & \colorbox{Yellow}{0.178} & \textcolor{red}{20h} & \textbf{0.0033} & - \\
            MobileNeRF$^{\pmb{\dagger}}$$^{\ddagger}$ & 25.91 & 0.825 & \colorbox{SkyBlue}{0.183} & \textcolor{red}{$>$48h} & \textbf{0.0029} & \textcolor{red}{201.5} \\
            Plenoxel$^{\pmb{\dagger}}$ & 26.29 & 0.839 & 0.210 & 24m & - & \textcolor{red}{19300} \\
            TensoRF & \colorbox{Yellow}{26.6} & 0.832 & 0.207 & 28m & \textcolor{red}{5.9} & \textcolor{red}{188} \\
            % \midrule[1pt] 
            \hline
            MobileR2L & 26.15 & \colorbox{YellowGreen}{0.966} & 0.187 & \textcolor{red}{$>$48h} & - & \textbf{8.3} \\
            NeRF-SR (2$\times$) & \colorbox{YellowGreen}{27.26} & 0.842 & \colorbox{YellowGreen}{0.103} & \textcolor{red}{$>$48h} & \textcolor{red}{39.1} & - \\ 
            RefSR-NeRF & 26.23 & \colorbox{SkyBlue}{0.874} & 0.243 & - & \textcolor{red}{8.5} & \textbf{38} \\
            Ours (2$\times$) & 26.20 & 0.822 & 0.241 & \textbf{150m} & \textbf{0.786} & \textbf{26} \\
            % Ours (4X) & 25.41 & 0.784 & 0.297 & \textbf{59m} & \textbf{0.163} & \textbf{15} \\
            % Ours (8X) & 21.30 & 0.584 & 0.475 & \textbf{15m} & \textbf{0.04} & \textbf{8} \\
            \bottomrule[1.5pt]
        \end{tabular}
        \caption{LLFF Dataset results.}
    \end{subtable}
    \end{center}
    \vspace{-15pt}
    \caption{
        Quantitative results and efficiency metrics on three different datasets.
        The first section of each table includes models that use implicit representation to the radiance field. 
        The middle section includes efficient models that use an explicit or hybrid representation to accelerate both training and inference. 
        The third section collects methods that utilize super sampling to improve both quality and speed including ours. 
        The first, second, and third best results of the quality metrics are highlighted in green, yellow, and blue. We use red text color when there is a clear disadvantage on either training time, rednering time or model size.
        $\pmb{\dagger}$ notes the method relies on customized kernels to achieve the training/rendering speed, while other methods are based on standard Python-based framework.
        $\ddagger$ notes the method requires at least 8 high-end GPUs to train.
        Our method achieves the best balance between training time, rendering speed and model size with on par accuracy against other efficient NeRF models. 
        % Note: Mip-NeRF training time is an early-stop version on RTX2080Ti GPU. Original training time is longer. Plenoxel uses customized CUDA. MobileNeRF need 8 V100 GPUs to train. 
    }
    \label{table:quantitative_results}
\end{table*}


==> tables/quantitative_results_v2.tex <==
\begin{table*}
    \begin{center}
    % NeRF-Synthetic results
    \begin{subtable}[t]{1.\textwidth}
        \centering
        \begin{tabular}{ ccccccc }
        \toprule[1.5pt]
        \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{PSNR$\uparrow$}} & \multirow{2}{*}{\textbf{SSIM$\uparrow$}} & \multirow{2}{*}{\textbf{LPIPS$\downarrow$}} & \textbf{Train} & \textbf{Render} & \textbf{Model} \\
        & & & & \textbf{Time} & \textbf{Time(s)} & \textbf{Size(MB)} \\
        \midrule[1pt] 
        NeRF \cite{mildenhall2020nerf} & 31.01 & 0.947 & 0.081 & \textcolor{red}{$\sim$35h} \qichen{consider using this: }\colorbox{red!30}{$\sim$35h} & \textcolor{red}{20} & 5 \\
        NSVF$^{\ddagger}$ \cite{liu2020nsvf} & 31.74 & 0.953 & 0.047 & \textcolor{red}{$>$48h} & \textcolor{red}{3} & - \\
        MipNeRF \cite{mipnerf} & \underline{33.09} & 0.961 & \underline{0.043} & \textcolor{red}{$\sim$35h} & - & - \\
        % \midrule[1pt] 
        \hline & \\[-1.5ex]
        % KiloNeRF$^{\pmb{\dagger}}$ & 31.00 & 0.950 & \textbf{0.030} & \textcolor{red}{$>$35h} & 0.026 & - \\
        SNeRG \cite{hedman2021snerg} & 30.38 & 0.950 & 0.05 & \textcolor{red}{$\sim$35h} & 0.012 & 86.8 \\
        % MobileNeRF$^{\pmb{\dagger}}$$^{\ddagger}$ & 30.90 & 0.947 & 0.062 & \textcolor{red}{$>$35h} & 0.0013 & \textcolor{red}{125.8} \\
        DVGO \cite{sun2021dvgo} & 31.95 & 0.958 & 0.053 & 14m & 0.44 & \textcolor{red}{612} \\
        Efficient-NeRF \cite{Hu_2022_CVPR_efficient_nerf} & 31.68 &  0.954 & \textbf{0.028} & 6h & 0.004 & \textcolor{red}{$\sim$3000} \\
        TensoRF \cite{chen2022tensorf} & \textbf{33.14} & \underline{0.963} & 0.049 & 18m & \textcolor{red}{1.4} & 71.8 \\
        % Plenoxel$^{\pmb{\dagger}}$ &  31.71 & 0.958 & 0.049 & 11m & 0.066 & \textcolor{red}{815} \\
        % DVGOv2$^{\pmb{\dagger}}$ & 32.76 & 0.962 & 0.046 & 7m & 0.254 & \textcolor{red}{612} \\
        % Instant-NGP$^{\pmb{\dagger}}$ & \textbf{33.18} & - & - & 5m & - & 16 \\
        % PlenOctrees & 31.71 & 0.958 & 0.053 & \textcolor{red}{$\sim$15h} & 0.006 & \textcolor{red}{1.97(GB)} \\ 
        % FastNeRF & 29.90 & 0.937 & 0.056 & - & 0.041 & \textcolor{red}{$>$7GB} \\
        \hline & \\[-1.5ex]
        MobileR2L \cite{cao2022mobiler2l} & 31.34 & \textbf{0.993} & 0.051 & \textcolor{red}{$>$35h} & - & 8.3 \\
        NeRF-SR \cite{wang2021nerf-sr} & 28.46 & 0.921 & 0.076 & \textcolor{red}{$>$35h} & \textcolor{red}{5.6} & - \\
        TF+SR(Ours) & 32.53 & 0.961 & 0.052 & 1.5h & 0.309 & 20 \\
        % Ours (4X) & 30.47 & 0.944 & 0.075 & \textbf{30m} & \textbf{0.077} & \textbf{13} \\
        % Ours (8X) & 27.27 & 0.902 & 0.142 & \textbf{16.5m} & \textbf{0.03} & \textbf{8}
        \bottomrule[1.5pt]
        \end{tabular}
        \vspace{5pt}
        \caption{NeRF Synthetic Dataset results.}
        \vspace{7pt}
    % }
    \end{subtable}
    % NSVF-Synthetic results
    \begin{subtable}[t]{1.\textwidth}
        \centering
        \begin{tabular}{ ccccccc }
            \toprule[1.5pt]
            \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{PSNR$\uparrow$}} & \multirow{2}{*}{\textbf{SSIM$\uparrow$}} & \multirow{2}{*}{\textbf{LPIPS$\downarrow$}} & \textbf{Train} & \textbf{Render} & \textbf{Model} \\
            & & & & \textbf{Time} & \textbf{Time(s)} & \textbf{Size(MB)} \\
            \midrule[1pt] 
            NeRF \cite{mildenhall2020nerf} & 30.81 & 0.952 & - & \textcolor{red}{$\sim$35h} & \textcolor{red}{$\sim$20} & $\sim$5 \\
            NSVF$^{\ddagger}$ \cite{liu2020nsvf} & 35.13 & \textbf{0.979} & - & \textcolor{red}{$>$48h} & \textcolor{red}{$\sim$3} & - \\
            \hline & \\[-1.5ex]
            % KiloNeRF$^{\pmb{\dagger}}$ & 33.37 & 0.970 & \textbf{0.020} & \textcolor{red}{$>$35h} & 0.026 & - \\
            DVGO \cite{sun2021dvgo} & 35.18 & \textbf{0.979} & - & $\sim$20m & - & \textcolor{red}{$\sim$600} \\
            TensoRF \cite{chen2022tensorf} & \textbf{36.52} & 0.959 & \textbf{0.027} & 15m & \textcolor{red}{1.4} & 74 \\
            \hline & \\[-1.5ex]
            TF+SR(Ours) & \underline{35.39} & \textbf{0.979} & \underline{0.032} & 1.5h & 0.302 & 26 \\
            % Ours (4X) & 32.04 & 0.958 & 0.059 & \textbf{30m} & \textbf{0.075} & \textbf{12} \\
            \bottomrule[1.5pt]
        \end{tabular}
        \vspace{5pt}
        \caption{NSVF Synthetic Dataset results.}
        \vspace{7pt}
    \end{subtable}
    \begin{subtable}[t]{1.\textwidth}
        \centering
        \begin{tabular}{ ccccccc }
            \toprule[1.5pt]
            \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{PSNR$\uparrow$}} & \multirow{2}{*}{\textbf{SSIM$\uparrow$}} & \multirow{2}{*}{\textbf{LPIPS$\downarrow$}} & \textbf{Train} & \textbf{Render} & \textbf{Model} \\
            & & & & \textbf{Time} & \textbf{Time(s)} & \textbf{Size(MB)} \\
            \midrule[1pt] 
            NeRF \cite{mildenhall2020nerf} & 26.5 & 0.811 & 0.250 & \textcolor{red}{$\sim$48h} & \textcolor{red}{33} & 5 \\
            \hline & \\[-1.5ex]
            SNeRG \cite{hedman2021snerg} & 25.63 & 0.818 & 0.183 & \textcolor{red}{$\sim$48h} & 0.036 & \textcolor{red}{310}\\
            NeX \cite{Wizadwongsa2021_NeX} & \underline{27.26} & \underline{0.904} & \underline{0.178} & \textcolor{red}{20h} & 0.0033 & - \\
            % MobileNeRF$^{\pmb{\dagger}}$$^{\ddagger}$ & 25.91 & 0.825 & 0.183 & \textcolor{red}{$>$48h} & 0.0029 & \textcolor{red}{201.5} \\
            % Plenoxel$^{\pmb{\dagger}}$ & 26.29 & 0.839 & 0.210 & 24m & - & \textcolor{red}{19300} \\r
            % FastNeRF & 26.04 & 0.856 & 0.085 & - & 0.005 & 57GB \\
            Efficient-NeRF \cite{Hu_2022_CVPR_efficient_nerf} & \textbf{27.39} & 0.912 & 0.082 & 4h & 0.005 & \textcolor{red}{4300} \\
            TensoRF \cite{chen2022tensorf} & 26.6 & 0.832 & 0.207 & 28m & \textcolor{red}{5.9} & \textcolor{red}{188} \\
            % \midrule[1pt] 
            \hline & \\[-1.5ex]
            MobileR2L \cite{cao2022mobiler2l} & 26.15 & \textbf{0.966} & 0.187 & \textcolor{red}{$>$48h} & - & 8.3 \\
            NeRF-SR \cite{wang2021nerf-sr} & \underline{27.26} & 0.842 & \textbf{0.103} & \textcolor{red}{$>$48h} & \textcolor{red}{39.1} & - \\ 
            RefSR-NeRF \cite{huang2023refsrnerf} & 26.23 & 0.874 & 0.243 & - & \textcolor{red}{8.5} & 38 \\
            TF+SR(Ours) & 26.20 & 0.822 & 0.241 & 2.5h & 0.786 & 26 \\
            % Ours (4X) & 25.41 & 0.784 & 0.297 & \textbf{59m} & \textbf{0.163} & \textbf{15} \\
            % Ours (8X) & 21.30 & 0.584 & 0.475 & \textbf{15m} & \textbf{0.04} & \textbf{8} \\
            \bottomrule[1.5pt]
        \end{tabular}
        \vspace{5pt}
        \caption{LLFF Dataset results.}
        \vspace{7pt}
    \end{subtable}
    \end{center}
    \vspace{-15pt}
    \caption{
        Quantitative results and efficiency metrics on three different datasets.
        The first section of each table includes the implicit MLP-based NeRF models.
        % use implicit representation to the radiance field. 
        The middle section are the excpiclit or hybrid NeRF that aim to have an improved rendering or training speed.
        % includes efficient models that use an explicit or hybrid representation to accelerate both training and inference. 
        The third section collects SR-based NeRF models including ours, which uses TensoRF (TF) as the NeRF backbone.
        % methods that utilize super sampling to improve both quality and speed including ours. 
        The best and second best results of each quantitative metrics are highlighted in \textbf{bold} and \underline{underline}.
        % The first, second, and third best results of the quality metrics are highlighted in green, yellow, and blue. 
        We highlight the result in \textcolor{red}{red} when there is a clear disadvantage on the efficiency metrics.
        % We only compare to models that do not rely on customized GPU kernels for a fair comparison on the model efficiency.
        % $\pmb{\dagger}$ notes the method relies on customized kernels to achieve the training/rendering speed, while other methods are based on standard Python-based framework.
        % TF stands for TensoRF which is the backbone NeRF model we use and we show the results for 2$\times$.
        $\ddagger$ notes the method requires at least 8 high-end GPUs to train.
        We report our model's results at SR rate 2$\times$.
        % as it achieves comparable quality to other state-of-the-art methods. 
        Our method produces \textbf{excellent quantitative results that is on par or only slightly less than the state-of-the-art} cross all the benchmarks.
        Our method further achieves \textbf{the best balance between training time, rendering speed and model size}, while other methods struggle to have good performance on these three metrics at the same time.
        % even when compared to other NeRF models that are designed to maximize efficiency.
        % against other efficient NeRF models. 
        % with \textbf{on par accuracy} 
        % Note: Mip-NeRF training time is an early-stop version on RTX2080Ti GPU. Original training time is longer. Plenoxel uses customized CUDA. MobileNeRF need 8 V100 GPUs to train. 
    }
    \label{table:quantitative_results}
\end{table*}


==> tables/quantitative_results_v3.tex <==
\begin{table*}
    \begin{center}
    % NeRF-Synthetic results
    \begin{subtable}[t]{.9\textwidth}
        \centering
        \begin{tabular}{ |m{2.6cm}|m{1cm}|m{1cm}|m{1cm}|m{1cm}|m{1.2cm}|m{1.25cm}| }
        \hline
        \multirow{3}{*}{\textbf{Method}} & \multicolumn{6}{c|}{NeRF-Synthesic} \\
        \cline{2-7}
        & \multirow{2}{*}{\textbf{PSNR$\uparrow$}} & \multirow{2}{*}{\textbf{SSIM$\uparrow$}} & \multirow{2}{*}{\textbf{LPIPS$\downarrow$}} & \textbf{Train} & \textbf{Render} & \textbf{Model} \\
        & & & & \textbf{Time} & \textbf{Time(s)} & \textbf{Size(MB)} \\
        \hline
        NeRF \cite{mildenhall2020nerf} & 31.01 & 0.947 & 0.081 & $\sim$35h & 20 & 5 \\
        \hline 
        MobileR2L \cite{cao2022mobiler2l} & 31.34 & \textbf{0.993} & 0.051 & $>$35h & - & 8.3 \\
        NeRF-SR \cite{wang2021nerf-sr} & 28.46 & 0.921 & 0.076 & $>$35h & 5.6 & - \\
        \hline
        TensoRF \cite{chen2022tensorf} & \textbf{33.14} & \underline{0.963} & 0.049 & 18m & 1.4 & 71.8 \\
        TF+SR(Ours) & 32.53 & 0.961 & 0.052 & 1.5h & 0.309 & 20 \\
        \hline
        \end{tabular}
        \vspace{5pt}
    \end{subtable}
    % NSVF-Synthetic results
    \begin{subtable}[t]{.9\textwidth}
        \centering
        \begin{tabular}{ |p{2.6cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1.2cm}|p{1.25cm}| }
            \hline
            \multirow{3}{*}{\textbf{Method}} & \multicolumn{6}{c|}{NSVF-Synthesic} \\
            \cline{2-7}
            & \multirow{2}{*}{\textbf{PSNR$\uparrow$}} & \multirow{2}{*}{\textbf{SSIM$\uparrow$}} & \multirow{2}{*}{\textbf{LPIPS$\downarrow$}} & \textbf{Train} & \textbf{Render} & \textbf{Model} \\
            & & & & \textbf{Time} & \textbf{Time(s)} & \textbf{Size(MB)} \\
            \hline
            NeRF \cite{mildenhall2020nerf} & 30.81 & 0.952 & - & $\sim$35h & $\sim$20 & $\sim$5 \\
            \hline
            TensoRF \cite{chen2022tensorf} & \textbf{36.52} & 0.959 & \textbf{0.027} & 15m & 1.4 & 74 \\
            TF+SR(Ours) & \underline{35.39} & \textbf{0.979} & \underline{0.032} & 1.5h & 0.302 & 26 \\
            \hline
        \end{tabular}
        \vspace{5pt}
    \end{subtable}
    \begin{subtable}[t]{.9\textwidth}
        \centering
        \begin{tabular}{ |p{2.6cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1.2cm}|p{1.25cm}| }
        \hline
        \multirow{3}{*}{\textbf{Method}} & \multicolumn{6}{c|}{LLFF} \\
        \cline{2-7}
        & \multirow{2}{*}{\textbf{PSNR$\uparrow$}} & \multirow{2}{*}{\textbf{SSIM$\uparrow$}} & \multirow{2}{*}{\textbf{LPIPS$\downarrow$}} & \textbf{Train} & \textbf{Render} & \textbf{Model} \\
        & & & & \textbf{Time} & \textbf{Time(s)} & \textbf{Size(MB)} \\
        \hline
        NeRF\cite{mildenhall2020nerf} & 26.5 & 0.811 & 0.250 & $\sim$48h & 33 & 5 \\
        \hline 
        MobileR2L\cite{cao2022mobiler2l} & 26.15 & \textbf{0.966} & 0.187 & $>$48h & - & 8.3 \\
        NeRF-SR\cite{wang2021nerf-sr} & \underline{27.26} & 0.842 & \textbf{0.103} & $>$48h & 39.1 & - \\ 
        RefSR-NeRF\cite{huang2023refsrnerf} & 26.23 & 0.874 & 0.243 & - & 8.5 & 38 \\
        \hline
        TensoRF\cite{chen2022tensorf} & 26.6 & 0.832 & 0.207 & 28m & 5.9 & 188 \\
        TF+SR(Ours) & 26.20 & 0.822 & 0.241 & 2.5h & 0.786 & 26 \\
        \hline
        \end{tabular}
        \vspace{7pt}
    \end{subtable}
    \end{center}
    \vspace{-15pt}
    \caption{
        Quantitative results and efficiency metrics on NeRF-Synthetic, NSVF-Synthetic and LLFF dataset.
        We compare to our baseline model, TensoRF, and other SR-based NeRF methods.
        We also list the vanilla NeRF's results for reference.
    }
    \label{table:quantitative_results}
\end{table*}



==> tables/sr_ratio_comparison.tex <==
\begin{table*}
    \begin{center} 
    \resizebox{0.75\textwidth}{!}{ 
    \begin{tabular}{ cccccccc }
        \toprule[1.5pt]
        \multirow{2}{*}{Dataset} & Upscale & PSNR & SSIM & LPIPS & Train & Render & Model \\
        & Ratio & & & & Time(m) & Time(ms) & Size(MB) \\
        \midrule[0.5pt] 
        \multirow{3}{*}{NeRF-Synthetic} 
        & 2x & 32.53 & 0.961 & 0.052 & 89 & 309 & 20 \\
        & 4x & 30.47 & 0.944 & 0.075 & 30 & 77 & 13 \\
        & 8x & 27.27 & 0.902 & 0.142 & 16.5 & 30 & 8 \\
        \midrule[0.5pt] 
        \multirow{3}{*}{NSVF-Synthetic} 
        & 2x & 35.39 & 0.979 & 0.032 & 92 & 302 & 26 \\
        & 4x & 32.04 & 0.958 & 0.059 & 30.5 & 75 & 12 \\
        & 8x & 27.93 & 0.911 & 0.119 & 16.5 & 29.6 & 9 \\
        \midrule[0.5pt] 
        \multirow{3}{*}{LLFF} 
        & 2x & 26.20 & 0.817 & 0.243 & 61 & 769 & 26 \\
        % & 4x & 24.83 & 0.750 & 0.328 & 34m & 0.317 & 15 \\
        & 4x & 25.41 & 0.784 & 0.297 & 57.5 & 165 & 15 \\
        & 8x & 21.30 & 0.584 & 0.475 & 15 & 40 & 8 \\
        \bottomrule[1.5pt]
    \end{tabular}}
    \end{center}
    \caption{Quantitative and efficiency metrics on NeRF-Synthetic, NSVF-Synthetic and LLFF datasets of our method.}
    \label{table:abalation_patch_aug}
\end{table*}

==> tables/synthetic_comparison.tex <==

\begin{table*}
    \begin{center} 
    \resizebox{0.95\textwidth}{!}{ 
    \begin{tabular}{ c|ccc|cccccc }
        \toprule[1.5pt]
        % \multirow{3}{*}{\textbf{Method}} 
        & \multicolumn{3}{c}{NSVF-Synthetic} & \multicolumn{6}{|c}{NeRF-Synthetic} \\
        \multirow{2}{*}{\textbf{Method}} 
        & \multirow{2}{*}{\textbf{PSNR}} & \multirow{2}{*}{\textbf{SSIM}} & \multirow{2}{*}{\textbf{LPIPS}}
        & \multirow{2}{*}{\textbf{PSNR}} & \multirow{2}{*}{\textbf{SSIM}} & \multirow{2}{*}{\textbf{LPIPS}} 
        & \textbf{Train} & \textbf{Render} & \textbf{Model} \\
        % & \multirow{2}{*}{\textbf{PSNR}} & \multirow{2}{*}{\textbf{SSIM}} & \multirow{2}{*}{\textbf{LPIPS}} & \textbf{Train} & \textbf{Render} & \textbf{Model} & \multirow{2}{*}{\textbf{PSNR}} & \multirow{2}{*}{\textbf{SSIM}} & \multirow{2}{*}{\textbf{LPIPS}} \\
        % & \textbf{Time} & \textbf{Time(s)} & \textbf{Size(MB)} & & & \\
        & & & & & & & \textbf{Time} & \textbf{Time(s)} & \textbf{Size(MB)} \\
        \midrule[1pt] 
        NeRF 
        & 30.81 & 0.952 & -
        & 31.01 & 0.947 & 0.081
        & \textcolor{red}{$\sim$35h} & \textcolor{red}{20} & 5 \\
        NSVF 
        & 35.13 & 0.979 & -
        & 31.74 & 0.953 & 0.047 
        & \textcolor{red}{$>$48h} & \textcolor{red}{3} & - \\
        MipNeRF 
        & - & - & -
        & 33.09 & 0.961 & 0.043 
        & \textcolor{red}{$\sim$35h} & - & - \\
        \hline
        DVGO 
        & 35.18 & 0.979 & - 
        & 31.95 & 0.957 & 0.053 
        & 22m & - & \textcolor{red}{612} \\
        TensoRF 
        & 36.52 & 0.959 & 0.027 
        & 33.14 & 0.963 & 0.049 
        & 18m & \textcolor{red}{1.4} & \textcolor{red}{71.8} \\
        Plenoxel 
        & - & - & - 
        & 31.71 & 0.958 & 0.049 
        & 11m & 0.066 & \textcolor{red}{815} \\
        KiloNeRF 
        & 33.37 & 0.97 & 0.020 
        & 31.00 & 0.950 & 0.03 
        & \textcolor{red}{$>$35h} & 0.026 & - \\
        MobileNeRF 
        & - & - & - 
        & 30.90 & 0.947 & 0.062 
        & \textcolor{red}{$>$35h} & 0.0013 & \textcolor{red}{125.8} \\
        % Instant-NGP \\
        % \midrule[1pt] 
        % PlenOctrees & 31.71 & 0.958 & 0.053 & \textcolor{red}{$\sim$15h} & 0.006 & \textcolor{red}{1.97(GB)} \\ 
        % FastNeRF & 29.90 & 0.937 & 0.056 & - & 0.041 & \textcolor{red}{$>$7GB} \\
        % SNeRG & 30.38 & 0.950 & 0.05 & \textcolor{red}{$\sim$35h} & 0.012 & \textcolor{red}{86.8} \\
        \hline
        MobileR2L 
        & - & - & - 
        & 31.34 & 0.993 & 0.051 
        & \textcolor{red}{$>$35h} & - & 8.3 \\
        NeRF-SR 
        & - & - & - 
        & 28.46 & 0.921 & 0.076 
        & \textcolor{red}{$>$35h} & TODO & - \\
        Ours (2X) 
        & 35.39 & 0.979 & 0.032 
        & 32.53 & 0.961 & 0.052 
        & \textbf{89m} & \textbf{0.309} & \textbf{20} \\
        Ours (4X) 
        & 32.04 & 0.958 & 0.059 
        & 30.47 & 0.944 & 0.075 
        & 30m & 0.077 & 13 \\
        \bottomrule[1.5pt]
    \end{tabular}}
    \end{center}
    \caption{Results on NeRF Synthetic Datset. The first section includes models that use a big MLP to represent the radiance field. The middle section includes efficient models that use an explicit or hybrid representation to accelerate both training and inference. The third section collects methods that utilize SR to improve both quality and speed including ours.  Our method achieves a great balance between training time, rendering speed and model size with on par accuracy against other efficient NeRF models. Note: Mip-NeRF training time is an early-stop version on RTX2080Ti GPU. Original training time is longer. Plenoxel uses customized CUDA. MobileNeRF need 8 V100 GPUs to train. We use red text color to highlight the part when there is a clear disadvantage of the work.}
    \label{table:nerf_synthetic_main}
\end{table*}

% \begin{table*}
%     \begin{center} 
%     \resizebox{0.7\textwidth}{!}{ 
%     \begin{tabular}{ ccccccc }
%         \toprule[1.5pt]
%         \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{PSNR}} & \multirow{2}{*}{\textbf{SSIM}} & \multirow{2}{*}{\textbf{LPIPS}} & \textbf{Train} & \textbf{Render} & \textbf{Model} \\
%         & & & & \textbf{Time} & \textbf{Time(s)} & \textbf{Size(MB)} \\
%         \midrule[1pt] 
%         NeRF & 30.81 & 0.952 & - & \textcolor{red}{$\sim$35h} & \textcolor{red}{$\sim$20} & $\sim$5 \\
%         NSVF & 35.13 & 0.979 & - & \textcolor{red}{$>$48h} & \textcolor{red}{$\sim$3} & - \\
%         \hline
%         DVGO & 35.18 & 0.979 & - & $\sim$20m & - & \textcolor{red}{$\sim$600} \\
%         TensoRF & 36.52 & 0.959 & 0.027 & 15m & \textcolor{red}{1.4} & \textcolor{red}{74} \\
%         KiloNeRF & 33.37 & 0.97 & 0.020 & \textcolor{red}{$>$35h} & 0.026 & - \\
%         \hline
%         Ours (2X) & 35.39 & 0.979 & 0.032 & 92m & 0.302 & 26 \\
%         Ours (4X) & 32.04 & 0.958 & 0.059 & 30.5m & 0.075 & 12 \\
%         \bottomrule[1.5pt]
%     \end{tabular}}
%     \end{center}
%     \caption{Results on NSVF Synthetic Datset. NSVF requires 8 GPUs to train.}
%     \label{table:nerf_synthetic_main}
% \end{table*}
